Is LLM-as-a-Judge Robust? Investigating Universal Adversarial Attacks on Zero-shot LLM Assessment

Large Language Models (LLMs) are powerful zero-shot assessors used in real-world situations such as assessing written exams and benchmarking systems. Despite these critical applications, no existing work has analyzed the vulnerability of judge-LLMs to adversarial manipulation. This work presents the first study on the adversarial robustness of assessment LLMs, where we demonstrate that short universal adversarial phrases can be concatenated to deceive judge LLMs to predict inflated scores. Since adversaries may not know or have access to the judge-LLMs, we propose a simple surrogate attack where a surrogate model is first attacked, and the learned attack phrase then transferred to unknown judge-LLMs. We propose a practical algorithm to determine the short universal attack phrases and demonstrate that when transferred to unseen models, scores can be drastically inflated such that irrespective of the assessed text, maximum scores are predicted. It is found that judge-LLMs are significantly more susceptible to these adversarial attacks when used for absolute scoring, as opposed to comparative assessment. Our findings raise concerns on the reliability of LLM-as-a-judge methods, and emphasize the importance of addressing vulnerabilities in LLM assessment methods before deployment in high-stakes real-world scenarios.

==> latex/temp.tex <==
\section{Zero-shot Assessment with LLMs}
As discussed by \citet{zhu2023judgelm, liusie2023zero}, there are two standard reference-free methods of prompting instruction-tuned LLMs for quality assessment:
\begin{itemize}
    \item \textbf{LLM Scoring} where an LLM is asked to assign a score to each considered text
    \vspace{-2mm}
    \item \textbf{LLM Comparative Assessment} where the system uses pairwise comparisons to determine which of two responses are better
\end{itemize}
%
For various assessment methods, we consider rankings tasks where given a query context $\mathbf d$  and a set of $N$ candidate responses $\mathbf x_{1:N}$, the objective is to determine the quality of each response, $s_{1:N}$. An effective LLM judge should predict scores for each candidate that match the ranking $r_{1:N}$ of the text's true quality. This section will further discuss the details of both comparative assessment (Section \ref{sec:comparative}) and absolute assessment (Section \ref{sec:absolute}). 

% With an appropriate prompt, instruction-tuned Large Language Models (LLMs) can be used in a zero-shot manner for assessment of natural language. Consider a context $\mathbf d$ (for example a text passage or dialogue) and a set of $N$ candidate responses, $\mathbf x_{1:N}$. For an attribute of interest (e.g., coherency, fluency, consistency, etc, ...), there exist true (human annotated) scores for the quality of each response, $s_{1:N}$. An effective LLM as a judge should be able to predict scores for each candidate response to give the same true ranking of the candidate responses, $r_{1:N}$.

% Popular LLM assessment approaches can be categorized in two groups: comparative assessment (Section \ref{sec:comparative}) and absolute assessment (Section \ref{sec:absolute}).


\subsection{Comparative Assessment} \label{sec:comparative}

Given the context $\mathbf d$ and two candidate responses, $\mathbf x_i$ and $\mathbf x_j$, an LLM prompted for comparative assessment, $\mathcal F$, is prompted to predict the probability that response $\mathbf x_i$ is better than response $\mathbf x_j$,
\begin{equation}
    p_{ij} = \mathcal F(\mathbf x_i, \mathbf x_j, \mathbf{d}) + (1-\mathcal F(\mathbf x_j, \mathbf x_i, \mathbf{d})),
\end{equation}
where two inferences passes of the model $\mathcal F$ are used to ensure that comparative assessment satisfies symmetry, such that $p_{ij}=p_{ji}$. These pair-wise probabilities can be used to obtain predicted assessment scores for each response $\mathbf x_{1:N}$, such that
\begin{equation} \label{eqn:comp-score}
    \hat s_n = \hat s(\mathbf x_n) = \frac{1}{N}\sum_{j=1}^N p_{nj}.
\end{equation}
With all the predicted scores, $\hat s_{1:N}$, the ranks $\hat r_{1:N}$ can be computed and evaluated with respect to the reference ranks $r_{1:N}$.
 
\subsection{Absolute Assessment} \label{sec:absolute}

When performing absolute assessment, the LLM, $\mathcal F$, is prompted to directly predict a score (e.g., the prompt requests the LLM to assess the quality of the text and give a score between 1-5). Here, two variants of absolute assessment can be applied. First, the score is the value directly predicted by the LLM,
\begin{equation}
    \hat s_n = \hat s(\mathbf x_n) = \mathcal{F}(\mathbf x_n, \mathbf d),.
\end{equation}
Alternatively, as proposed by G-Eval \textbf{ref)} the expectation of all possible scores can be computed when there is access to the predicted logits from the LLM,
\begin{equation} \label{eqn:abs-score}
    \hat s_n  = \hat s(\mathbf x_n) =  \sum_{k=1:K} kP_{\mathcal F}(k|\mathbf{x}_n, \mathbf c),
\end{equation}
where $K$ is the maximum score indicated in the prompt and the predicted probabilities for the possible scores $1:K$ are normalized to be real probabilities, $\sum_{k=1:K}P_{\mathcal F}(k|\mathbf{x}_n, \mathbf c) = 1$ and $P_{\mathcal F}(k|\mathbf{x}_n, \mathbf c)\geq0$, $\forall n$.

As with comparative assessment, the predicted scores, $\hat s_{1:N}$,  can be converted to ranks $\hat r_{1:N}$.




\section{Adversarial Assessment Attacks}
\subsection{Attack Objective}
An adversary aims to modify the input text $\mathbf x$ to fool the assessment system into predicting a higher score. In the traditional definition of an adversarial attack, an adversarial example ${\bm\delta}$ is a small perturbation on an input $\mathbf x$, that causes a change in the output prediction of a system, $\mathcal F$,
\begin{equation}
    \mathcal F(\mathbf{x}+\bm\delta) \neq \mathcal F(\mathbf x),
\end{equation}
where $+$ represents a perturbation in the input text space and the notion of a perturbation being `small' is typically captured by some proxy function for human perception, $\mathcal G(\mathbf{x}, \mathbf{x}+\bm\delta)\leq\epsilon$. However, in the context of attacking an assessment system, the adversary aims to perturb their input, $\mathbf x_i$ such that the predicted rank (as determined from the predicted scores defined in Equation \ref{eqn:comp-score} or \ref{eqn:abs-score}) of the attacked sample is the best relative to all the other unattacked samples, $\mathbf x_{1:N}$. If we let $\hat r^{\prime}_i$ represent the rank of the attacked sample $\mathbf x_i+\bm\delta$, when no other sample in $\mathbf x_{1:N}$ is perturbed,
\begin{equation}
    \hat r^{\prime}_i(\bm\delta) = \texttt{rank}_i\left(\hat s(\mathbf x_1), \hdots, \hat s(\mathbf x_i+\bm\delta), \hdots, \hat s(\mathbf x_N),  \right )
\end{equation}
then the adversarial objective for candidate $i$ is one that minimizes the predicted rank relative to the other unattacked candidates,
\begin{equation} \label{eqn:adv-obj}
    \bm\delta^*_i = \argmin_{\bm\delta} (\hat r^{\prime}_i(\bm\delta)).
\end{equation}
Nevertheless, in the assessment setting, it is not practical for candidates to individually learn an adversarial example $\bm\delta^*_i$ to fool an LLM system into predicting a high score. It is simpler for candidates to use a \textit{universal} adversarial example $\bm\delta^*$ that can be applied in a simple manner to any candidate's text $\mathbf x$ and always boosts the rank predicted by the LLM assessment system. For a training set of $M$ samples of contexts and $N$ candidate texts, $\left\{(\mathbf c^{(m)}, \mathbf x^{(m)}_{1:N})\right\}_{m=1}^M$ an optimal adversarial example is one that minimizes the average rank, where the average is with respect to both the samples $M$ and each candidate text being attacked separately in turn, $N$
\begin{align} \label{eqn:avg-rank}
    \bm\delta^* &= \argmin_{\bm\delta} (\bar r(\bm\delta))\\
    \bar r(\bm\delta) &= \frac{1}{NM}\sum_m\sum_n \hat r^{\prime (m)}_n(\bm\delta).
\end{align}
To ensure that the universal attack $\bm\delta$ is simple for candidates to apply, we let $\mathbf x+\bm\delta$ represent a concatenation of the attack phrase words of $\bm\delta$ to the original text $\mathbf x$, i.e. $\mathbf x+\bm\delta = x_1, \hdots, x_{|\mathbf x|}, \delta_1,\hdots, \delta_L $, where $|\mathbf x|$ is the number of words in the original text $\mathbf x$ and $L$ is the number of words in the attack phrase $\bm\delta$. 

\subsection{Practical Attack Approach}

In this work, we use a \textit{greedy} search to learn the universal attack phrase~\footnote{We also carried out experiments using the Greedy Coordinate Gradient (GCG) attack \textbf{ref} to learn the universal attack phrase, but this approach was found to be not as effective as the greedy search process. Results for GCG experiments are provided in Appendix \textbf{todo}.}. For a vocabulary, $\mathcal V$ the greedy search looks for the next most effective adversarial word to append iteratively,
\begin{align}
    \delta^*_{l+1} = \argmin_{\delta\in\mathcal V} (\bar r(\delta^*_{1:l} + \delta)).
\end{align}
However, in practice it can be computationally too expensive to compute the average rank (as in Equation \ref{eqn:avg-rank}) in each iteration of the greedy search, so instead two relaxations are made in the practical search process. First, only select candidate texts are used in each training sample: for absolute assessment, only a single candidate response, $\mathbf x_a$ of $\mathbf{x}_{1:N}$ is used for each training sample $m$ and a single pair of responses $\mathbf x_a$ and $\mathbf x_b$ is used in the attack for comparative assessment from each training sample $m$. Second, the greedy search process is modified to maximise the average (over all training samples $m$) predicted score for the selected samples ($\mathbf x_a$, $\mathbf x_b$) as opposed to minimizing the rank. The algorithms for the practical greedy search attack on comparative assessment and absolute assessment systems are given in Algorithm \ref{alg:comp} and Algorithm \ref{alg:abs} respectively.


\begin{algorithm} 
\caption{Greedy Search Attack for Comparative Assessment} \label{alg:comp}
\begin{algorithmic} 
\Require $\left\{(\mathbf c^{(m)}, \mathbf x^{(m)}_{1:N})\right\}_{m=1}^M$ \Comment{Training Data}
\Require $\mathcal F()$ \Comment{Target Model}
\State $\bm\delta^* \gets \text{ empty string}$

\For{$l=1:L$}
    \State $\delta^*_l\gets \text{ none}$
    \State $q^*\gets 0$ \Comment Initialize best score
    \For{$\delta\in\mathcal V$}
        \State $\bm\delta \gets \bm\delta^*+\delta$ \Comment{trial attack phrase}
        \State $q\gets 0$
        \For{$m=1:M$}
            \State $s_a\gets \mathcal F(\mathbf x^{(m)}_a+\bm\delta, \mathbf{x}^{(m)}_b, \mathbf c^{(m)})$
            \State $s_b\gets \mathcal F(\mathbf x^{(m)}_a, \mathbf{x}^{(m)}_b+\bm\delta, \mathbf c^{(m)})$
            \State $q\gets q+s_a+s_b$
        \EndFor
        \If{$q>q^*$}
            \State $q^*\gets q$ 
            \State $\delta^*_l\gets \delta$ \Comment{Update best attack word}
        \EndIf
    \EndFor
    \State $\bm\delta^*\gets \bm\delta^*+\delta^*_l$ \Comment{Update attack phrase}
\EndFor
\end{algorithmic}
\end{algorithm}


\begin{algorithm} 
\caption{Greedy Search Attack for Absolute Assessment}\label{alg:abs}
\begin{algorithmic} 
\Require $\left\{(\mathbf c^{(m)}, \mathbf x^{(m)}_{1:N})\right\}_{m=1}^M$ \Comment{Training Data}
\Require $\mathcal F()$ \Comment{Target Model}
\State $\bm\delta^* \gets \text{ empty string}$

\For{$l=1:L$}
    \State $\delta^*_l\gets \text{ none}$
    \State $q^*\gets 0$ \Comment Initialize best score
    \For{$\delta\in\mathcal V$}
        \State $\bm\delta \gets \bm\delta^*+\delta$ \Comment{trial attack phrase}
        \State $q\gets 0$
        \For{$m=1:M$}
            \State $s\gets \mathcal F(\mathbf x^{(m)}_a+\bm\delta, \mathbf c^{(m)})$
            \State $q\gets q+s$
        \EndFor
        \If{$q>q^*$}
            \State $q^*\gets q$ 
            \State $\delta^*_l\gets \delta$ \Comment{Update best attack word}
        \EndIf
    \EndFor
    \State $\bm\delta^*\gets \bm\delta^*+\delta^*_l$ \Comment{Update attack phrase}
\EndFor
\end{algorithmic}
\end{algorithm}
%% ALGORITHMS HERE


